A New World in the Depths of Microcrypt: Separating OWSGs and Quantum Money from QEFID

While in classical cryptography, one-way functions (OWFs) are widely regarded as the "minimal assumption," the situation in quantum cryptography is less clear. Recent works have put forward two concurrent candidates for the minimal assumption in quantum cryptography: One-way state generators (OWSGs), postulating the existence of a hard search problem with an efficient verification algorithm, and EFI pairs, postulating the existence of a hard distinguishing problem. Two recent papers [Khurana and Tomer STOC'24; Batra and Jain FOCS'24] showed that OWSGs imply EFI pairs, but the reverse direction remained open. In this work, we give strong evidence that the opposite direction does not hold: We show that there is a quantum unitary oracle relative to which EFI pairs exist, but OWSGs do not. In fact, we show a slightly stronger statement that holds also for EFI pairs that output classical bits (QEFID). As a consequence, we separate, via our oracle, QEFID, and one-way puzzles from OWSGs and several other Microcrypt primitives, including efficiently verifiable one-way puzzles and unclonable state generators. In particular, this solves a problem left open in [Chung, Goldin, and Gray Crypto'24]. Using similar techniques, we also establish a fully black-box separation (which is slightly weaker than an oracle separation) between private-key quantum money schemes and QEFID pairs. One conceptual implication of our work is that the existence of an efficient verification algorithm may lead to qualitatively stronger primitives in quantum cryptography.

==> proofs/efid-emulator.tex <==
\begin{proof}
Suppose not, and there exists an oracle-aided quantum algorithm $\adv$ making $r(\secp)\in O(2^{\frac{\secp}{50}})$ queries to the oracle $U_{S_\secp}$\footnote{We can assume without loss of generality that $\adv$ only queries $U_{S_\secp}$ and not the oracles $U_{S_{\secp'}}$ for $\secp'\neq\secp$ since the $U_{S_{\secp'}}$ for $\secp'\neq\secp$ are sampled independently from the current computational indistinguishability game.}, such that 
\begin{align*}
\EE_{O\gets\oracle}\left[\Pr_{s\gets D^O_0(1^\secp)}[\adv^{O,\qpspace}(1^\secp,s)=1]-\Pr_{s\gets D^O_1(1^\secp)}[\adv^{O, \qpspace}(1^\secp,s)=1]\right]> 2^{-\frac{2\secp}{25}}.
\end{align*}

Then, by \Cref{prop:reflect-emulate-efid} and letting $t(\secp)=2r(\secp)^2\cdot (4\cdot 2^{{2\secp}/{25}})^2$, there exists an algorithm $\badv$ that only queries $\qpspace$ and obtains the following distinguishing advantage
\begin{align}\nonumber
&\EE_{O\gets\oracle}\left[\Pr_{s\gets D^O_0(1^\secp)}[\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]-\Pr_{s\gets D^O_1(1^\secp)}
[\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]\right]\\ \label{eq:emulation-contradiction} &> \frac{1}{2^{\frac{2\secp}{25}}}-\frac{1}{4\cdot2^{\frac{2\secp}{25}}}-\frac{1}{4\cdot2^{\frac{2\secp}{25}}}=\frac{1}{2\cdot2^{\frac{2\secp}{25}}}=2^{-\frac{2\secp}{25}-1}\in \Omega\left(2^{-\frac{2\secp}{25}}\right).
\end{align}
% Note that by linearity of expectation,
% \begin{align}
%     &\EE_{O\gets\oracle}\left[\Pr_{s\gets D^O_0(1^\secp)}[\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]-\Pr_{s\gets D^O_1(1^\secp)}
% [\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]\right]\\ 
% &=\EE_{O\gets\oracle}\left[\Pr_{s\gets D^O_0(1^\secp)}[\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]\right]-\EE_O
% \end{align}
which is the same as saying for two uniformly random subsets of size $2^{\frac{\secp}{2}}$ $S,W\subset \bin^\sec\setminus\{0^\sec\}$, and uniformly random strings  $s\gets S$, and $u\gets\bin^\sec$,
\begin{align}
    \Expct_{S,s}\left[\Pr_\badv[\badv^{\qpspace}(1^\secp,\ket{S-}^{\otimes t}\otimes\ket{s})=1]\right]-\Expct_{W,u}\left[\Pr_\badv[\badv^{\qpspace}(1^\secp,\ket{W-}^{\otimes t}\otimes\ket{u})=1]\right]\in\Omega\left(2^{-\frac{2\secp}{25}}\right).\label{eq:emulation-contradiction-1}
\end{align}
%where $S,W\subset \bin^\sec\setminus\{0^\sec\}$ be two uniformly random subsets of size $2^{\frac{\secp}{2}}$, $s\gets S$, and $u\gets\bin^\sec$.
% \mor{Why we can change into $|W\rangle$? Also, QPSPACE oracle to $\cB$ is forgotten here?}\amit{I added the explanation and included QPSPACE oracle.}
\Cref{eq:emulation-contradiction-1} follows from the observation that

$\Expct_O[\Pr_{s\gets D^O_0(1^\secp)}[\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]]$ can be written as $\Expct_{S,s}\left[\Pr_\badv[\badv^{\qpspace}(1^\secp,\ket{S-}^{\otimes t}\otimes\ket{s})=1]\right]$ and $\Expct_O[\Pr_{s\gets D^O_0(1^\secp)}[\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]]$ can be written as $\Expct_{W,u}\left[\Pr_\badv[\badv^{\qpspace}(1^\secp,\ket{W-}^{\otimes t}\otimes\ket{u})=1]\right]$ where $S,W,s,u$ are distributed as mentioned above, and hence by linearity of expectation,
\begin{align}
&\EE_{O\gets\oracle}\left[\Pr_{s\gets D^O_0(1^\secp)}[\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]-\Pr_{s\gets D^O_1(1^\secp)}
[\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]\right]\\
&=\Expct_{S,s}\left[\Pr_\badv[\badv^{\qpspace}(1^\secp,\ket{S-}^{\otimes t}\otimes\ket{s})=1]\right]-\Expct_{W,u}\left[\Pr_\badv[\badv^{\qpspace}(1^\secp,\ket{W-}^{\otimes t}\otimes\ket{u})=1]\right]. 
\end{align}


However, note that
\begin{equation}\label{eq:t-bound}
    t(\secp)=2r(\secp)^2 (4\cdot 2^{\frac{2\secp}{25}})^2\in O(2^{\frac{2\secp}{50}}\cdot2^{\frac{4\secp}{25}})=O(2^\frac{9\secp}{50}).
\end{equation}


Combining \Cref{eq:t-bound} with \Cref{lem:EFID-trace-distance}, 
\mor{I do not understand how to use \cref{lem:EFID-trace-distance} here. In \cref{lem:EFID-trace-distance}, one is $S$ and the other is $W$, while
here both are $S$.}\amit{Yeah I need to change the $S$ to $W$ for one of the distributions. I have added a step. Is it better?}
we conclude that for some constant $c$, and $\secp$ large enough
% \begin{align}
%     &\EE_{O\gets\oracle}\left[\Pr_{s\gets D^O_0(1^\secp)}[\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]-\Pr_{s\gets D^O_1(1^\secp)} [\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]\right]\\
% &\leq 2^{-\frac{\secp}{2}+1} + \sqrt{c\frac{2^{\frac{9\secp}{50}}}{{2^{\frac{\secp}{2}+1}}}}=2^{-\frac{\secp}{2}+1} + \sqrt{c}2^{-\frac{4\secp}{25}}\leq (1+\sqrt{c})2^{-\frac{4\secp}{25}}\in o(2^{-\frac{2\secp}{25}}),%\label{eq:emulation-contradiction-2}
% \end{align}
\begin{align}
&\Expct_{S,s}\left[\Pr_\badv[\badv^{\qpspace}(1^\secp,\ket{S-}^{\otimes t}\otimes\ket{s})=1]\right]-\Expct_{W,u}\left[\Pr_\badv[\badv^{\qpspace}(1^\secp,\ket{W-}^{\otimes t}\otimes\ket{u})=1]\right]\\
% &\EE_{O\gets\oracle}\left[\Pr_{s\gets D^O_0(1^\secp)}[\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]-\Pr_{s\gets D^O_1(1^\secp)}
% [\badv^{\qpspace}(1^\secp,\ket{S_\secp-}^{\otimes t},s)=1]\right]\\
&\leq 2^{-\frac{\secp}{2}+1} + \sqrt{c\frac{2^{\frac{9\secp}{50}}}{{2^{\frac{\secp}{2}+1}}}}=2^{-\frac{\secp}{2}+1} + \sqrt{c}2^{-\frac{4\secp}{25}}\leq (1+\sqrt{c})2^{-\frac{4\secp}{25}}\in o(2^{-\frac{2\secp}{25}}),%\label{eq:emulation-contradiction-2} 
\end{align}
which contradicts the bound in \Cref{eq:emulation-contradiction-1}, thereby completing the proof.
%Clearly, since $q(\secp)$ is polynomial, \Cref{eq:emulation-contradiction,eq:t-bound} together contradict the bound in \Cref{lem:EFID-trace-distance} which completes the proof. 

% Next, in order to show contradiction to the previous equation, we will show that for any polynomial $t(\secp)$
% \[\{\ket{S-}^{\otimes t},s\}_{s\gets D^{S_\secp}_0(1^\secp), S_\secp\xleftarrow{\$} \binom{\{0,1\}^\secp}{2^{\frac{\secp}{4}}}}\approx_s \{\ket{S-}^{\otimes t},s\}_{s\gets D^{S_\secp}_1(1^\secp), S_\secp\xleftarrow{\$} \binom{\{0,1\}^\secp}{2^{\frac{\secp}{4}}}}\]
\end{proof}

==> proofs/efid-vs-qmoney.tex <==
\begin{proof}
    Suppose there exists a $(q,\epsilon)$-fully black-box construction of a private-key quantum money scheme $\QQ=(\kgen,\mint,\verify)$ from a \qefid pair
    with a corresponding reduction $\reduction$.
    
    Let $\oracle$ be the distribution over oracles defined in \Cref{def:S-oracle} and consider a random $O\gets\oracle$. Let $(D^O_0,D^O_1)$ be the oracle-aided \qefid pair from \Cref{con:efi}. By construction, $(D^O_0,D^O_1)$ is efficiently sampleable and, by \Cref{prop:statistical-farness}, it satisfies statistical farness as required by \Cref{def:efi}.

    By \Cref{thm:statistical-break-quantum-money}, there exists a polynomial-query quantum adversary $\adv$ that breaks $\QQ$ relative to any $O\in\oracle$ and, in particular, relative to a random $O\gets\oracle$ with probability 1. Therefore, by the correctness of $\reduction$, it must hold that
    \[
        \left| \Pr_{x\gets D^O_0(1^\sec)}[\reduction^{\adv,O}(1^\secp,x)=1]-\Pr_{x\gets D^O_1(1^\sec)}[\reduction^{\adv,O}(1^\secp,x)=1]\right| \geq \epsilon(\sec)
    \]
    for infinitely many $\sec\in\NN$.

    Let $p:=p(\kappa)$ be the polynomial bound on the query complexity of $\adv$ and $p':=p'(\kappa)$ be the polynomial bound on the query complexity of $\verify$. We can replace $\reduction$ by an algorithm $\widetilde{\reduction}$ that makes $p\cdot p'\cdot q$ queries to $O$, while not accessing $\adv$ at all, by simulating the queries to $\adv$ and $\adv$'s queries to $\verify$ in by itself (in fact, as we already mention, our attack $\adv$ queries $O$ only and does not query the verification oracle, hence, in our case there are no ``nested'' queries to $\verify$ that must be simulated).

    By \Cref{lem:computational-indistinguishability-EFID-pair}, if $\epsilon(\sec)\in \omega (2^{-\sec/51}) \subset\omega (2^{-\sec/50})$, such an algorithm $\widetilde{\reduction}$ must perform $\omega(2^{\sec/50})$ queries to $O$. Hence $p\cdot p'\cdot q\in\omega(2^{\sec/50})$ and, since $p$ and $p'$ are polynomials, $q\in\omega(2^{\sec/51})$.
\end{proof}


==> proofs/gentle-search.tex <==

\begin{proof}%\amit{Changed to mixed state formalism and not pure states.}
    Our algorithm applies the gentle search procedure devised by Aaronson~\cite[Lemma 15]{Shadow2}. Assuming, w.l.o.g., that $|K|$ is a power of 2, Aaronson's gentle search is a binary-search type of algorithm, that, at every iteration, divides the given collection of POVM elements into two halves and applies the quantum OR-tester, described below, on each to identify the half consisting of the target key, and proceeds recursively therein.

    The OR-tester~\cite[Corollary 3.1]{HLM17} is a test which, given a collection of binary-valued POVMs $\zeta_1,\dots,\zeta_m$ and a state $\rho$ (one copy thereof) distinguishes between the following two cases: \begin{enumerate}%[label=(\roman*)]
        \item There exists $i\in [m]$ such that $\Tr(\zeta_i\rho)\geq \gamma_1$, \label{it:condition1} and
        \item $\Expct_{i\gets [m]}[\Tr(\zeta_i\rho)]< \gamma_2$\label{it:condition2},
    \end{enumerate}
    for $\gamma_1>1/2$ and $\gamma_1>\gamma_2$, the choice of which affects the complexity of the test and its advantage. 

Using such a tester, Aaronson~\cite[Lemma 14]{Shadow2} demonstrates given a collection of binary-valued POVMs $\tilde{\zeta}_1,\dots,\tilde{\zeta}_m$ and a state $\rho$, how to construct a tester that distinguishes between the following for any $0\leq c\leq 1$ and $\epsilon>0$,
    \begin{enumerate}[label=(\roman*)]
        \item There exists $i\in [m]$ such that $\Tr(\tilde{\zeta}_i\rho)\geq c$, \label{it:condition1-aar} and
        \item $\forall i\in [m]$, $\Tr(\tilde{\zeta}_i\rho)< c-\epsilon$\label{it:condition2-aar}.
    \end{enumerate}
    %Aaronson~\cite[Lemma 14]{Shadow2} demonstrates how to boost the advantage of such a tester given sufficiently many copies of the input state and make it work for any $\gamma_1>\gamma_2$ and not necessarily $\gamma>1/2$. 
    Specifically, %given binary-valued POVMs $\tilde{Tau}_1,\ldots,\tilde{\zeta}_m$ and state $\rho$ satisfying \Cref{it:condition,it:condition2} with some $\gamma_1,\gamma_2$ such that $\gamma_1>\gamma_2$,
     he considers the amplified binary-valued POVMs $\{\zeta_i\}_i$ acting on $\rho^{\otimes \ell}$ for $\ell:=O(\frac{\log(m)}{\epsilon^2})$ such that \footnote{$\zeta_i$ runs $\tilde{\zeta}_i$ on $\rho$ $\ell$ times and accepts if $\zeta_i$ outputs accept at least $c-\frac{\epsilon}{2}$ times.} for the amplified POVMs and the state $\rho^{\otimes \ell}$, the OR-tester condition holds with $\gamma_1=1-\frac{1}{m}$ in \Cref{it:condition1} and $\gamma_2-\frac{1}{m}$ in \Cref{it:condition2}. Then, he runs the OR-tester of~\cite{HLM17} for the POVMs $\zeta_1,\ldots,\zeta_m$ for the state $\rho^{\otimes \ell}$, and further amplifies it such that his test is able to distinguish \Cref{it:condition1-aar} and \Cref{it:condition2-aar} with success probability $1-\eta$ using a total of $O(\log(1/\eta)\log^3 m/\epsilon^2)$ copies of $\rho$. Evidently, such a test with $\eta=\delta\cdot \log|K|$ suffices to instantiate the binary search described above, to obtain overall success probability $1-\delta$ with $t$ copies of the input state.

    Most importantly to us is the fact that the only place in Aaronson's gentle search where the POVMs are used is the OR-tester component. The OR-tester by Harrow et al.~\cite{HLM17} applies a variant of Marriott-Watrous gap-amplification procedure~\cite{MW05} to implement the POVM $\Pi=\sum_{k} \Pi_k$. Specifically, it consists of applying the projective measurements $\Lambda_0=\sum_k \Pi_k\otimes (Q\proj{k}Q^{-1})$ and $\Lambda_1=I\otimes \proj{0}$ on the input state, in an alternating fashion, where $Q$ denotes QFT over $\ZZ_{|K|}$.

     As noted by Chen et al.~\cite[Remark 5.3]{CCS24}, when the POVM elements $\{\Pi_k\}_k$ are projectors implementable by polynomial-query $\qpspace$-aided quantum circuits in polynomial space, then also the POVM $\Lambda_0$ may be implemented by a polynomial-query
    $\qpspace$-aided quantum circuit. We can generalize the remark (\cite[Remark 5.3]{CCS24}) for arbitrary POVM elements $\{\Pi_k\}_k$ implementable by polynomial-query $\qpspace$-aided quantum circuits in polynomial space.
    This is because every polynomial space implementable oracle-aided binary-valued POVM and in particular $\Pi_k$ for every $k$, can be implemented using a polynomial space implementable oracle-aided unitary $U_k$ acting on some $n+r$ qubits where the last $r$ qubits are additional ancillae initialized to zero (where $r\in \poly$ is an upper bound on the polynomial space needed to implement $\{\Pi_k\}_k$), followed by measuring the last qubit in the computational basis, and then accept if the outcome is $1$ else fail. Clearly, $\{U_k^\perp \left( I\otimes\ketbra{1}{1}\right) U_k\}_k$ has the same acceptance statistics for a state $\rho\otimes \ketbra{0^{\otimes r}}{0^{\otimes r}}$ as that of $\{\Pi_k\}_k$ on $\rho$, 
    \ifnum\submission=0
        because
        \begin{align}
            \Tr[\Pi_k\rho]=\Tr[\left( I\otimes\ketbra{1}{1}\right)U_k \left( \rho\otimes \ketbra{0^{\otimes r}}{0^{\otimes r}}\right) U_k^\perp]=\Tr[U_k^\perp \left( I\otimes\ketbra{1}{1}\right) U_k\left(\rho\otimes \ketbra{0^{\otimes r}}{0^{\otimes r}}\right)],
        \end{align}
    \fi
    and therefore by~\cite[Remark 5.3]{CCS24}, it is possible to implement the POVM $\Lambda_0$ by a polynomial-query
    $\qpspace$-aided quantum circuit.
    
    To conclude, it is possible to perform the gentle search algorithm from~\cite{Shadow2} in our setting, where the POVMs make a polynomially-bounded access to $\qpspace$. Its correctness follows by the analysis done in~\cite{HLM17,Shadow2} as outlined above. For futher details, we refer the reader to the aforementioned works.
\end{proof}

==> proofs/qmoney-attack.tex <==

\subsection{Proof of \texorpdfstring{\Cref{lem:qmoney-attack}}{Lemma 7.4}}
\label{sec:qmoney-attack-proof}


Clearly, $m'(\kappa)\in \poly(\kappa)$ since $\mu(\kappa)$ and $m(\kappa)$ are inverse polynomial function and polynommial function of $\kappa$ respectively. Therefore, $\adv$ is polynomial-query.

The rest of the proof is dedicated to analyze the success probability of $\adv$ in the forging game against $\QQ$.

For any $\kappa\in\NN$, $k\in\bin^\kappa$ and $n(\kappa)$-qubit state $\rho$, define
\begin{align*}
    &a_\V(k,\rho):=\Pr[\widetilde{\verify}(k,\rho,\tau)=1], && a_\VM(k,k'):=\Pr[\VM(k,k',\tau)=1],\\
    &\$(k):=\mint^O(k), && \text{and}\quad (\widetilde{\$}(k),\tau'):=\widetilde{\mint}(k,\tau),
\end{align*}
where $\widetilde{\$}(k)$ and $\tau'$ can be potentially entangled. %$\Tr(\cdot)_2$ denotes tracing out the second register.
% \mor{$\widetilde{\mint}$ outputs $\tau'$ as well, so $\widetilde{\$}(k)\coloneqq\widetilde{\mint}(k,\tau)$ means that $\widetilde{\$}(k)$ also contains $\tau'$.}\amit{Yeah it should not contain $\tau'$. Is it better now?}
% \mor{yes.}

\begin{proposition}\label{prop:av-avm}
    For any $\kappa\in\NN$ and $k,k'\in\bin^\kappa$, it holds that
    $$|a_\VM(k,k') - a_\V(k,{\$}(k'))|\leq \mu/\kappa.$$%\amit{$\mu$ change: was $1/\kappa$}
\end{proposition}
\begin{proof}
%Let $T_1,T_2$ be the input registers and $D$ be the output register for the quantum algorithm $\tilde{\mint}(\cdot,\cdot)$ .
Let $(\widetilde{\$}(k'),\tau')\gets \widetilde{\mint}(k',\tau)$. By \Cref{eq:mint-to-tilde-qmoney}, $\TD[(\widetilde{\$}(k'),\tau'),\$(k')\otimes \tau]\leq \frac{\mu}{\kappa}$. 
Hence,  
$|a_\VM(k,k') - a_\V(k,{\$}(k'))|$ is the same as
\[
|\Pr[\widetilde{\verify}(k,\widetilde{\$}(k'),\tau')=1]-\Pr[\widetilde{\verify}(k,{\$}(k'),\tau)=1]|\leq \frac{\mu}{\kappa}.
\]

    %\tamer{TODOTODOTODO}
\end{proof}

In the following claim, we establish a connection between the acceptance probabilities (in fact, the differences therein) by the verification algorithm $\verify$ and its emulated version, namely $\widetilde{\verify}$.

\begin{proposition}\label{prop:a-gap}
    For any $\kappa\in\NN$, $k,k'\in\bin^\kappa$ and $n(\kappa)$-qubit state $\rho$,
    \begin{equation*}
          \left||a_\V(k,\rho) - a_\VM(k,k')| - \left|\Pr[\verify^O(k,\rho) = 1] - \Pr[\verify^O(k,\$(k')) = 1]\right|\right| \leq 3\mu/\kappa.
    \end{equation*}
\end{proposition}

\begin{proof}
    %Denote $\delta = |\Pr[\verify^O(k,\rho) = 1] - \Pr[\verify^O(k,\$(k')) = 1]|$.

    By \Cref{eq:verify-to-tilde-qmoney}, %with the triangle inequality,\mor{where do you use triangle inequality?}
    \begin{align}\label{eq:tratata-first}
         \left| \Pr[\verify^O(k,\rho)=1] - a_\V(k,\rho) \right| =\left| \Pr[\verify^O(k,\rho)=1]- \Pr[\widetilde{\verify}(k,\rho,\tau)=1] \right| \leq \frac{\mu}{\kappa}.
    \end{align}
    %\mor{$\widetilde{\verify}^O$ should be typo.}

    Further, using \Cref{eq:tratata-first} for $\rho=\$(k')$, 
    along with \Cref{prop:av-avm} 
    %\mor{where do you use \cref{eq:mint-to-tilde-qmoney}?}
    and triangle inequality, we have
    \begin{align}\nonumber
         &\left| \Pr[\verify^O(k,\$(k'))=1] - a_\VM(k,k') \right|\\\nonumber
         &\leq\left| \Pr[\verify^O(k,\$(k'))=1] - a_\V(k,{\$}(k')) \right| + \mu/\kappa&\text{By \Cref{prop:av-avm}.}\\\nonumber
%         &\leq\left| \Pr[\verify^O(k,\$(k'))=1]- a_\V(k,\$(k')) \right|
        %+\left| a_\V(k,\$(k')) -a_\V(k,\widetilde{\$}(k')) \right|
%        + \mu/\kappa\\
        &\leq {\mu}/{\kappa}+{\mu}/{\kappa}&\text{By \Cref{eq:tratata-first}.}\\
        &= {2\mu}/{\kappa}.\label{eq:verify_mint-to-tilde-qmoney}
    \end{align}
Combining  \Cref{eq:tratata-first,eq:verify_mint-to-tilde-qmoney} and by triangle inequality, we get
\begin{align}\nonumber
    &|a_\V(k,\rho) - a_\VM(k,k')|\leq |\Pr[\verify^O(k,\rho) = 1] - \Pr[\verify^O(k,\$(k')) = 1]|+3\mu/\kappa\\\nonumber
    &|\Pr[\verify^O(k,\rho) = 1] - \Pr[\verify^O(k,\$(k')) = 1]|\leq |a_\V(k,\rho) - a_\VM(k,k')| + 3\mu/\kappa.
\end{align}
    The proposition follows by combining the last two equations.

    %\amit{I do not follow the second line here.}\amit{Firstly there is a problem with triangle inequality, I think this is arising because we are working in absolute value in the claim, we just need to say that the difference of probabilities is $\delta$ then the absolute value of the difference between $\delta$ and the difference of the a's is at most $3/\kappa$. Secondly, and more importantly, it seems you are writing $a_\VM(k,k')$ as $a_\V(k,\widetilde{\$}(k'))$, which is not true since in $\VM$ you would use $\tau'$ and in $\V$ you would use $\tau$ and $\tau\neq \tau'$ though $\tau\approx\tau'$}
\end{proof}

%By definition, for any pair of keys $k,k'\in\bin^\kappa$ and $\tau$ as defined in \Cref{eq:tau-def}, 
%\begin{align}
%a_\V(k,\tilde{\$}(k'))=\Pr[\VM(k,k',\tau)=1].
%\end{align}




% Hence, \Cref{eq:verify_mint-to-tilde-qmoney} implies that
% \begin{align}\label{eq:vm-qmoney}
%     \left| \Pr[\ver^{O}(k,\mint^{O}(k'))=1] -\Pr[\VM(k,\tau,k',\tau)=1] \right|\leq \frac{2}{\kappa}
% \end{align}

%\amit{Here.}






% Therefore,
% \begin{align}
%     &|\Pr[\ver(k',\$(k'))=1]- \Pr[\ver(k',\tilde{\$}))=1]|\\
%     &\leq |\Pr[\ver(k',\$(k'))=1]- \Pr[{\widetilde{\ver}}(k',\$(k'))=1]|+|\Pr[{\widetilde{\ver}}(k',\$(k'))=1]-\tilde{b}_{k'}|\\
%     &+|\tilde{b}_{k'}- \Pr[{\widetilde{\ver}}_k(\tilde{\$}))=1]|+|\Pr[{\widetilde{\ver}}_k(\tilde{\$}))=1]-\Pr[\ver(k',\tilde{\$}))=1]|\\
%     &\leq \frac{1}{\kappa}+|\Pr[{\widetilde{\ver}}(k',\$(k'))=1]-\tilde{b}_{k'}|+\frac{1}{\kappa}+\frac{1}{\kappa}.&\text{By \Cref{eq:verify-to-tilde-qmoney,eq:qmoney-sdp trick}}\\
%     &=|\Pr[{\widetilde{\ver}}(k',\$(k'))=1]-\tilde{b}_{k'}|+\frac{3}{\kappa}.
% \end{align}
We fix $\kappa\in\NN$ and let $k^*\gets\kgen(1^\sec)$ be the key sampled by the challenger in the unforgeability game and $\$^*\gets\mint(k^*)$ be the corresponding input to $\adv$. Let $E$ denote the event that the estimators $\estver$ and $\estvm$ run by $\adv$ were successful. That is, $E$ occurs if and only if \Cref{eq:estimate-shadow-tomography-private-quantum-money,eq:estimate-shadow-tomography-vm-private-quantum-money} hold for the the values $\{b_\V(k,\$^*)\}$ and $\{b_\VM(k,k')\}$ that are output in Steps~\ref{it:estimator-ver} and~\ref{it:estimator-vm} of $\adv$, respectively. By the guarantee of \cref{thm:shadow-tomography-estimates}, 
\begin{align}\label{eq:E-success-probability}
    \Pr[E]\geq1-\frac{2}{2^\kappa}.
\end{align}

In the next claim, we rely on the guarantee from shadow tomography to show that, if a state minted under a key $k'$ behaves like the input state $\$^*$ w.r.t. verification under any arbitrary key $k$, then the key $k'$ exhibits an estimate $b_\V(k,\$^*)$ that is similar to the estimate $b_\VM(k,k')$.

\begin{proposition}\label{prop:b-gap}
    Conditioned on $E$, for any $\kappa\in\NN$ and $k,k'\in\bin^\kappa$
    \begin{equation}
        \left|| b_\V(k,\$^*) - b_\VM(k,k') |-|\Pr[\verify^O(k,\$^*)] - \Pr[\verify^O(k,\$(k')]|\right|\leq  5\mu/\kappa. 
    \end{equation}
\end{proposition}
\begin{proof}
It is enough to show that conditioned on $E$,
\begin{equation}\label{eq:simpler-b-gap}
\left||b_\V(k,\$^*) - b_\VM(k,k')| -|a_\V(k,\$^*)-a_\VM(k,k')|\right|\leq 2\mu/\kappa,
\end{equation}
because then by \Cref{prop:a-gap} for $\rho=\$^*$, and triangle inequality,
\begin{align}
&\left||b_\V(k,\$^*) - b_\VM(k,k')| - \left|\Pr[\verify^O(k,\$^*)] - \Pr[\verify^O(k,\$(k')]\right|\right|\\
&\leq \left||b_\V(k,\$^*) - b_\VM(k,k')|-|a_\V(k,\$^*)-a_\VM(k,k')|\right|+3\mu/\kappa\\
&\leq 2\mu/\kappa+3\mu/\kappa=5\mu/\kappa,
\end{align}
which concludes the proof of the proposition. Therefore, we prove \Cref{eq:simpler-b-gap}.




    Note that conditioned on $E$, by its definition, it holds that
        \begin{align}\label{eq:estimate-shadow-tomography-both-private-quantum-money-algorithm}
        |b_\V(k,\$^*)-a_\V(k,\$^*)|\leq \frac{\mu}{\kappa} && \text{and} &&
        |b_\VM(k,k')-a_\VM(k,k')|\leq \frac{\mu}{\kappa},
    \end{align}%\amit{Tamer, the last equation is incorrect I think because $a_\V(k,\widetilde{\$}(k'))$ is defined with respect to a fresh $\tau$ but on the other hand,   $b_\VM(k,k')$ is an estimate for the verification $\widetilde{\verify}$ on $\widetilde{\$}(k')$ with respect to $\tau'$ which is a slightly disturbed version of  $\tau$ that is obtained at the end of $\widetilde{\mint}(k,\tau)$. Hence in order to claim this equation, we need to invoke \Cref{eq:mint-to-tilde-qmoney}. }\amit{I have written the fix in the next comment using \Cref{eq:mint-to-tilde-qmoney}, but it would change the bound on \Cref{eq:simpler-b-gap} to $4\mu/\kappa$ and hence the bound on the proposition to $11\mu/\kappa$. Therefore we have to change the parameters from $10\mu/\kappa$ to $22\mu/\kappa$.}
    and, consequently, by triangle inequality on \Cref{eq:estimate-shadow-tomography-both-private-quantum-money-algorithm}, we get
    \begin{align}
        &\left|b_\V(k,\$^*)-b_\VM(k,k')\right|
        \leq \left|a_\V(k,\$^*)-a_\VM(k,k')\right|+\frac{2\mu}{\kappa}.\\
        &\left|a_\V(k,\$^*)-a_\VM(k,k')\right|\leq \left|b_\V(k,\$^*)-b_\VM(k,k')\right|+\frac{2\mu}{\kappa}.
    \end{align}
    The last two equations together imply \Cref{eq:simpler-b-gap}.
    %\amit{
%Note that by \Cref{eq:mint-to-tilde-qmoney},
% \begin{align}
%     &|a_\V(k,\widetilde{\$}(k'))-a_\VM(k,k')|\\
%     &=\left|\Pr[\widetilde{\verify(k,\widetilde{\$}(k'),\tau)}]-\Pr[\widetilde{\verify(k,\widetilde{\$}(k'),\tau')}]\right|\\
%     &\leq \TD\left[(\widetilde{\$}(k')\otimes \tau),(\widetilde{\$}(k')\tau'\right]\\
%     &\leq \TD\left[(\widetilde{\$}(k')\otimes \tau),(\$(k')\otimes \tau)\right]+\TD\left[(\$(k')\otimes \tau),(\widetilde{\$}(k')\tau'\right]\\
%     &\leq \TD\left[\widetilde{\$}(k'),\$(k')\right]+\frac{\mu}{\kappa}&\text{By \Cref{eq:mint-to-tilde-qmoney}}\\
%     &\leq \TD\left[(\widetilde{\$}(k'),\tau'),(\$(k')\otimes \tau)\right]+\frac{\mu}{\kappa}\\
%     &\leq 2\frac{\mu}{\kappa}&\text{By \Cref{eq:mint-to-tilde-qmoney}}.\label{eq:vm-v-diff}
% \end{align}
% Note that conditioned on $E$, by its definition, it holds that
% \begin{align}\label{eq:estimate-shadow-tomography-both-private-quantum-money-algorithm-comment}
%         |b_\V(k,\$^*)-a_\V(k,\$^*)|\leq \frac{\mu}{\kappa} && \text{and} &&
%         |b_\VM(k,k')-a_\VM(k,k')|\leq \frac{\mu}{\kappa},
%     \end{align}
% Combining this with \Cref{eq:vm-v-diff}, we conclude that conditioned on the event $E$,
% \begin{align}\label{eq:estimate-shadow-tomography-both-private-quantum-money-algorithm-comment-2}
%         |b_\V(k,\$^*)-a_\V(k,\$^*)|\leq \frac{\mu}{\kappa} && \text{and} &&
%         |b_\VM(k,k')-a_\V(k,\widetilde{\$}(k'))|\leq \frac{3\mu}{\kappa},
%     \end{align}
%     and, consequently, by triangle inequality on \Cref{eq:estimate-shadow-tomography-both-private-quantum-money-algorithm-comment-2}, we get
%     \begin{align}
%         &\left|b_\V(k,\$^*)-b_\VM(k,k')\right|
%         \leq \left|a_\V(k,\$^*)-a_\V(k,\widetilde{\$}(k'))\right|+\frac{4\mu}{\kappa}.\\
%         &\left|a_\V(k,\$^*)-a_\V(k,\widetilde{\$}(k'))\right|\leq \left|b_\V(k,\$^*)-b_\VM(k,k')\right|+\frac{4\mu}{\kappa}.
%     \end{align}
%     The last two equations together imply \Cref{eq:simpler-b-gap}.(but with bound $4\mu/\kappa$ instead of $2\mu/\kappa$.)
% }

%     \begin{align}
%         &\leq \Pr[\verify^O(k,\$^*)] - \Pr[\verify^O(k,\$(k')] + \frac{3}{\kappa}+\frac{2}{\kappa}&\text{(By \Cref{prop:a-gap})}\\
%         &=\Pr[\verify^O(k,\$^*)] - \Pr[\verify^O(k,\$(k')]+\frac{5}{\kappa}.\nonumber%label{eq:est-tilde-distance}
% \end{align}

%     \begin{align}\nonumber
%         &\left||a_\V(k,\$^*)-a_\V(k,\widetilde{\$}(k'))|-|b_\V(k,\$^*)-b_\VM(k,k')|\right|\\\nonumber
%         &\leq \left|a_\V(k,\$^*)-a_\V(k,\widetilde{\$}(k'))-b_\V(k,\$^*)+b_\VM(k,k')\right|\\\nonumber
%         &\leq \left|a_\V(k,\$^*) - b_\V(k,\$^*)\right|+\left|a_\V(k,\widetilde{\$}(k'))-b_\VM(k,k')\right|\\
%         &\leq \frac{1}{\kappa}+\frac{1}{\kappa}=\frac{2}{\kappa}.\label{eq:est-tilde-distance}
% \end{align}



% Now, letting $\delta = \Pr[\verify^O(k,\$^*)] - \Pr[\verify^O(k,\$(k')]$, and by \Cref{eq:est-tilde-distance} with \Cref{prop:a-gap}, we conclude that
%  \begin{align*}
%     &\left|\delta-|b_\V(k,\$(k*))-b_\VM(k,k')|\right|\\
%     &\leq \left|\delta-|a_\V(k,\$^*)-a_\V(k,\widetilde{\$}(k'))|\right|\\&\quad +\left||a_\V(k,\$^*)-a_\V(k,\widetilde{\$}(k'))|-|b_\V(k,\$^*)-b_\VM(k,k')|\right|\\
%     &\leq  \frac{3}{\kappa}+\frac{2}{\kappa}=\frac{5}{\kappa}.
% \end{align*}
\end{proof}



In particular, applying \Cref{prop:b-gap} with $k'=k^*$, it follows that, conditioned on $E$
\begin{equation}
|b_\V(k,\$^*)-b_\VM(k,k^*)|\leq 5\mu/\kappa.
\end{equation}
for all $k\in\bin^\kappa$. Hence, conditioned on $E$, there exists $k'$ such that \Cref{eq:constraint-finder} is satisfied, in which case $\adv$ does not abort. From this point on, we assume $E$ occurs. By \Cref{eq:E-success-probability}, this incurs only a negligible loss in the success probability.

Let $k''$ be the $k'$ that $\adv$ finds in step~\ref{step:find}. In the following claim, we show that a quantum money state minted under $k''$, namely $\$(k'')$, verifies under $k^*$ with good probability.

\begin{claim}
    Conditioned on $E$,
    \begin{equation}\label{claim:single-success-probability}
        \Pr[\verify^O(k^*,\$(k''))=1]\geq \mu\left(1 - 10/\kappa\right).
    \end{equation}
\end{claim}

\begin{proof}
    By our construction of $\adv$ (step~\ref{step:find}), it holds that
    \begin{align*}
        |{b}_\V(k^*,\$^*)-{b}_\VM(k^*,k'')|\leq 5\mu/\kappa.
    \end{align*}
    By the above and \Cref{prop:b-gap}, we conclude that
    \begin{align*}
        &|\Pr[\verify^O(k^*,\$^*)=1]-\Pr[\verify^O(k^*,\$(k''))=1]|\\\label{eq:final-frontier} &\leq  |b_\V(k^*,\$^*)-b_\VM(k^*,k'')| +5\mu/\kappa \leq 10\mu/\kappa,
    \end{align*}
    which implies the inequality in the claim by the $\mu$-correctness of the scheme.
\end{proof}

Having shown that a single money state $\$(k'')\gets\mint^O(k'')$ passes verification under $k^*$, all that separates us from showing that $\adv$ is successful is a simple concentration bound, using which we argue that $m'=\ceil{2{\kappa}m/\left(\mu\left(1-{10}/{\kappa}\right)\right)}$ such states contain at least $m+1$ states that pass verification, with good enough probability.

Let $r$ denote the number of money states among the $m'$ states that $\adv$ outputs that pass verification under $k^*$. By \Cref{claim:single-success-probability}, $\Expct[r]\geq \left(\mu\left(1-{10}/{\kappa}\right)\right)\cdot m' \geq 2\kappa m$. Thus, by Hoeffding's inequality,
\begin{align*}
    &\Pr[r\leq m] \leq \Pr[|r - \Expct[r]| \geq \kappa m] \leq 2e^{-2\kappa^2 m^2/m'} \leq 2e^{-2\kappa m\cdot \left(\mu\left(1-{10}/{\kappa}\right)\left(\frac{m}{2m+\mu(1-10/\kappa)}\right)\right)}\\
    &\leq 2e^{-2\kappa m\cdot \left(\mu\left(1-{10}/{\kappa}\right)/4\right)}
    =2e^{-\kappa \frac{n\kappa^{10}}{2\mu^4}\cdot \left(\mu\left(1-{10}/{\kappa}\right)\right)}=2e^{-\frac{\kappa^{11}}{2\mu^3} \left(1-{10}/{\kappa}\right)},
\end{align*}
which is negligible.
This, together with \Cref{eq:E-success-probability}, completes the proof of \Cref{lem:qmoney-attack}. %\tamer{only if $\mu=1$}\amit{Corrected for every inverse polynomial $\mu$.}}




==> proofs/qpspace-inverse.tex <==
\begin{proof}
    The algorithm computes the description of the Turing machine $M'$ that acts as follows. $M'$ runs $M$ for $t$ steps to obtain the gates of the circuit $C$ and then inverts them one by one starting from the last gate (without printing or storing all the intermediate gates), to obtain the inverse circuit $C^{-1}$. Let $t'$ denote the runtime of $M'$. The algorithm then calls the $\qpspace$ oracle with $(\rho, M', t')$.
    
    The runtime of $M'$ is at most $O(t + |C|^2)$ (note that inversion is applied, w.l.o.g., to constant-size gates), where, $|C|$ is the size of $C$, i.e., the number of gates. Since $|C|$ is obviously bounded by $t$, it holds that $t'=O(t^2)$ and, in particular, its description as an integer is at most a constant factor by that of $t$. The description size of $M'$ is larger than that of $M$ by an additive $O(\log |C| + \log t)$. Hence, our simulation algorithm requires a single polynomial-size query.%\amit{Tamer, it was polynomial query initially but I think you meant a polynomial-size query, so I changed.}
\end{proof}

==> proofs/reflect-general.tex <==
\begin{proof}
    The corollary is obtained by applying \cref{thrm:reflect-jls} $m$ times to replace the reflection oracles with copies of the corresponding states, one at a time. Let $q_j$ be the number of queries made by $\adv$ to the oracle $\reflect_{\psi_j}$ (it holds $\sum_j q_j = q$). We denote by $\badv_j$ a quantum algorithm that is given access to $\reflect_{\psi_{j+1}},\dots,\reflect_{\psi_m}$ and takes $\ket{\psi_1}^{\otimes \ell},\dots,\ket{\psi_j}^{\otimes \ell}$ as input (besides $\ket{\phi}$). We define $\badv_0$ to behave identically to $\adv$. For $j>0$, we let $\badv_j$ be the algorithm obtained by applying \cref{thrm:reflect-jls} to $\badv_{j-1}$, to replace $\reflect_{\psi_{j}}$ with the input $\ket{\psi_j}^{\otimes \ell}$, where the input state to $\badv_{j-1}$ (denoted by $\ket{\phi}$ in the theorem's statement) is $\ket{\phi}\otimes\ket{\psi_1}^{\otimes \ell}\otimes\dots\otimes \ket{\psi_{j-1}}^{\otimes \ell}$. Due to the theorem, we know that the trace distance between the outcome of $\badv_j$ and that of $\badv_{j-1}$ is $q_j{2}/\sqrt{\ell+1}$ and, hence, the corollary holds for $\badv=\badv_m$.
\end{proof}

==> proofs/reflect-to-project.tex <==
\begin{proof}
        The required $R^c_{\phi}$-aided quantum algorithm on an input quantum state  $\ket{\psi}$ in input register $\mathsf{W}$ does the following.
        \begin{enumerate}
            \item Initializes a qubit-register $\mathsf{T}$ to the state $\ket{-}_\mathsf{T}$.
            \item Queries the oracle $R^c_{\phi}$ with $\mathsf{W}$ as the target register and $\mathsf{T}$ as the control register.
            \item Runs the Hadamard gate $H$ on register $\mathsf{T}$.
            \item Measures $\mathsf{T}$ in the computational basis.
            \item Output the input register $\mathsf{W}$ and declare success if the measurement outputs $0$ else declare failure.
        \end{enumerate}
    For the analysis, note that for any input state $\ket{\psi},$ there exists a pure state $\ket{\phi}^\perp$ which is orthogonal to $\ket{\phi}$, and complex numbers $a,b$ such that $|a|^2+|b|^2=1$ and $\ket{\psi}=a\ket{\phi}+b\ket{\phi}^\perp$. Therefore,
        \begin{align*}
            |\ip{\psi}{\phi}|^{2}=|a|^2, 1-|\ip{\psi}{\phi}|^{2}=|b|^2.
        \end{align*}
    Hence, note that the state on registers $\mathsf{W},\mathsf{T}$ after the oracle query is
        \begin{align*}
            R^c_{\phi}(\ket{\psi}_\mathsf{W}\otimes \ket{-}_\mathsf{T})&=a\cdot R^c_{\phi}(\ket{\phi}_W\otimes \ket{-}_\mathsf{T})+b\cdot R^c_{\phi}(\ket{\phi}^\perp_\mathsf{W}\otimes \ket{-}_T)\\
            &=a\cdot\ket{\phi}_\mathsf{W}\otimes \ket{+}_\mathsf{T}+ b\cdot\ket{\phi}^\perp_\mathsf{W}\otimes \ket{-}_\mathsf{T}.
        \end{align*}
    Therefore the state on registers $\mathsf{W},\mathsf{T}$ before the measurement is
        \begin{align*}
            a\cdot\ket{\phi}_\mathsf{W}\otimes \ket{0}_\mathsf{T}+ b\cdot\ket{\phi}^\perp_\mathsf{W}\otimes \ket{1}_\mathsf{T}.
        \end{align*}
    Hence with probability $|a|^2=|\ip{\psi}{\phi}|^{2}$, the measurement outcome is $0$, i.e. the algorithm succeeds, and the resulting post-measured state on $\mathsf{W}$ is $\ket{\phi}_\mathsf{W}$, and with probability $|b|^2=1-|\ip{\psi}{\phi}|^{2}$, the measurement outcome is $1$, i.e. the algorithm fails.
\end{proof}

==> proofs/statistical-farness.tex <==

\begin{proof}
Let $S=\{S_\sec\}_\secp$ be the fixed randomness corresponding to the oracle $O$ (see \cref{def:S-oracle}). Fix $\sec\in\NN$ and let, for any $x\in\bin^\sec$, $p_x^0$ and $p_x^1$ denote the probabilities that $D_0^O(1^\secp)$ and, respectively, $D_1^O(1^\secp)$ output $x$.
Then,
\begin{align*}
&\SD(D_0^O(1^\secp),D_1^O(1^\secp))=\frac{1}{2}\sum_{x\in\bit^\secp}|p_x^0-p_x^1|\\
&\quad =\frac{1}{2}\sum_{x\in S}|p_x^0-p_x^1|+\frac{1}{2}\sum_{x\notin S}|p_x^0-p_x^1| =\frac{1}{2}\sum_{x\in S}\left|\frac{1}{2^{\sec/2}}-\frac{1}{2^\secp}\right|
+\frac{1}{2}\sum_{x\notin S}\frac{1}{2^\secp}\\
&\quad =\frac{1}{2}\cdot 2^{\sec/2}\cdot \frac{2^{\sec/2}-1}{2^\secp}+\frac{1}{2}\cdot(2^\secp-2^{\sec/2})\cdot \frac{1}{2^\secp} =1-\frac{1}{2^{\sec/2}},
\end{align*}
which is overwhelming in the security parameter $\secp$.
\end{proof}

==> proofs/statistical-lemma.tex <==
\begin{proof}
    Observe that the distribution on the r.h.s. in the trace distance
    satisfies 
    \begin{equation}\label{eq:W-W'}
    \TD\left[\left\{\ket{W-}^{\otimes t}
    \otimes\ket{u}\right\}_{W,u},\left\{\ket{W'-}^{\otimes t}\ket{u'}\right\}_{W',u'}\right]< 2^{-\frac{\secp}{2} + 1},
    \end{equation}
    where r.h.s distribution $(W',u')$ is sampled by first sampling $u'$ uniformly at random from $\{0,1\}^\secp$, and then sampling $W'$ as a uniformly random subset over $\bin^\sec\setminus\{0^\sec\}$ of size $2^{\frac{\secp}{2}}$ conditioned on $u'\notin W'$. \Cref{eq:W-W'} holds since a random subset of size $2^{\frac{\secp}{2}}$ does not contain a fixed string $u'$ except with probability ${2^{{\secp}/{2}}}/{(2^\secp-1)}< 2^{1-{\secp}/{2}}$. It is enough to bound, then, the trace distance between $\{\ket{S-}\otimes \ket{s}\}_{S,s}$ and $\{\ket{W'-}\otimes\ket{u'}\}_{W',u'}$.

    Next, observe that the l.h.s. distribution in the lemma's statement can be sampled as follows: Sample a uniform $s\gets\bin^\sec$, then a uniform subset $S\subset\bin^\sec\setminus\{0^\sec\}$ of size $2^{\frac{\secp}{2}}$ that contains $s$. On the other hand, $u'$ and $W'$ may be sampled by choosing $u'$ uniformly, then a uniformly random subset $W''$ containing $u'$, and then defining $W' = W''\cup\{w\}\setminus\{u'\}$ for a uniformly random $w\gets \bin^\sec\setminus W''$.
    
    Note that such $W'',u'$ distribute identically to $S,s$. Hence, by an averaging argument, it is enough to show that for any fixed $s\in\bin^\sec$ and $S\subset\bin^\sec\setminus\{0^\sec\}$ such that $s\in S$ and any fixed $w\in \bin^\sec\setminus S$, the following holds
    \[
        \TD(\ket{S-}^{\otimes t}\ket{s},\ket{W'-}^{\otimes t}\ket{s}) = \TD(\ket{S-}^{\otimes t},\ket{W'-}^{\otimes t}),
    \]
    where $W'=S\cup\{w\}\setminus \{s\}$. Since $\ket{S-}^{\otimes t}$ and $\ket{W'-}^{\otimes t}$ are pure states, the trace distance is simply
    \begin{align}\nonumber
    &\sqrt{1-\langle S-| W'-\rangle^{2t}}
    =\sqrt{1-\left(\frac{1}{2} + \frac{1}{2}\cdot \sqrt{1-\frac{1}{2^{\frac{\secp}{2}}}}\right)^{2t}}\\\nonumber
    &\quad \leq \sqrt{1-\left(\frac{1}{2} + \frac{1}{2}\cdot \left(1-\frac{1}{2^{\frac{\secp}{2} +1}}\right)\right)^{2t}}=\sqrt{1-\left(1-\frac{1}{2^{\frac{\secp}{2} +2}}\right)^{2t}}\\%\nonumber
    &\quad\leq \sqrt{1-\left(1-\frac{2t}{2^{\frac{\secp}{2} +2}}\right)}
    =\sqrt{\frac{t}{2^{\frac{\secp}{2}+1}}}.\label{eq:S-W'}
    \end{align}
    The proof is complete by combining \Cref{eq:W-W',eq:S-W'}.
\end{proof}
